Optical--to--X-ray emission in low-absorption AGN: Results from the Swift-BAT 9 month catalogue

(Abridged) We present simultaneous optical--to--X-ray spectral energy distributions (SEDs) from Swift's X-ray and UV--optical telescopes (XRT and UVOT) for a well-selected sample of 26 low-redshift (z<0.1) AGN from the Swift/BAT 9-month catalogue, the largest well-studied, hard X-ray selected survey of local AGN to date. Our subsample consists of AGN with low intrinsic X-ray absorption (N_H<10^22 cm^-2) and minimal spectral complexity, to more accurately recover the intrinsic accretion luminosity in these sources. We perform a correction for host galaxy contamination in all available UVOT filter images to recover the intrinsic AGN emission, and estimate intrinsic dust extinction from the resultant nuclear SEDs. Black hole mass estimates are determined from the host-galaxy 2MASS K-band bulge luminosity. Accretion rates determined from our SEDs are on average low (Eddington ratios <~ 0.1) and hard X-ray bolometric corrections cluster at ~10-20, in contrast with the higher values seen for quasars. An average SED for the 22 low accretion rate (Eddington ratio < 0.1) objects is presented, with and without correction for intrinsic extinction. We do not find a correlation of optical--to--X-ray spectral index with Eddington ratio, regardless of the optical reference wavelength chosen for defining the spectral index. The low accretion rates and bolometric corrections found for this representative low-redshift sample are of particular importance for studies of AGN accretion history.

==> abstract <==
We present simultaneous optical--to--X-ray spectral energy distributions (SEDs) from Swift's X-ray and UV--optical telescopes (XRT and UVOT) for a well-selected sample of 26 low-redshift (z<0.1) active galactic nuclei (AGN) from the Swift/Burst Alert Telescope (BAT) 9-month catalogue, the largest well-studied, hard X-ray selected survey of local AGN to date.  Our subsample consists of AGN with low intrinsic X-ray absorption (N_{H}<10^{22} cm^{-2}) and minimal spectral complexity, to more accurately recover the intrinsic accretion luminosity in these sources.  We perform a correction for host galaxy contamination in all available UVOT filter images to recover the intrinsic AGN emission, and estimate intrinsic dust extinction from the resultant nuclear SEDs.  Black hole mass estimates are determined from the host-galaxy 2MASS K-band bulge luminosity.  Accretion rates determined from our SEDs are on average low (Eddington ratio \lambda_{Edd} <~ 0.1) and hard X-ray bolometric corrections cluster at ~10--20, in contrast with the higher values seen for quasars.  An average SED for the 22 low accretion rate (\lambda_{Edd}<0.1) objects is presented, with and without correction for extinction.  Significant dust reddening is found in some objects despite the selection of low N_{H} objects, emphasising the complex relationship between these two types of absorption.  We do not find a correlation of optical--to--X-ray spectral index with Eddington ratio, regardless of the optical reference wavelength chosen for defining the spectral index.  An anti-correlation of bolometric correction with black hole mass may reinforce `cosmic downsizing' scenarios, since higher bolometric corrections at low mass would boost accretion rates in local, lower mass black holes.  We also perform a basic analysis of the UVOT-derived host galaxy colours for our sample and find hosts cluster near the `green valley' of the colour-magnitude diagram, with possibly a handful of hosts with bluer colours.  The low accretion rates and bolometric corrections found for this representative low-redshift sample are of particular importance for studies of AGN accretion history.

